Predicting Defective Lines Using a Model-Agnostic Technique

Defect prediction models are proposed to help a team prioritize source code areas files that need Software QualityAssurance (SQA) based on the likelihood of having defects. However, developers may waste their unnecessary effort on the whole filewhile only a small fraction of its source code lines are defective. Indeed, we find that as little as 1%-3% of lines of a file are defective. Hence, in this work, we propose a novel framework (called LINE-DP) to identify defective lines using a model-agnostic technique, i.e., an Explainable AI technique that provides information why the model makes such a prediction. Broadly speaking, our LINE-DP first builds a file-level defect model using code token features. Then, our LINE-DP uses a state-of-the-art model-agnostic technique (i.e.,LIME) to identify risky tokens, i.e., code tokens that lead the file-level defect model to predict that the file will be defective. Then, the lines that contain risky tokens are predicted as defective lines. Through a case study of 32 releases of nine Java open source systems, our evaluation results show that our LINE-DP achieves an average recall of 0.61, a false alarm rate of 0.47, a top 20%LOC recall of0.27, and an initial false alarm of 16, which are statistically better than six baseline approaches. Our evaluation shows that our LINE-DP requires an average computation time of 10 seconds including model construction and defective line identification time. In addition, we find that 63% of defective lines that can be identified by our LINE-DP are related to common defects (e.g., argument change, condition change). These results suggest that our LINE-DP can effectively identify defective lines that contain common defectswhile requiring a smaller amount of inspection effort and a manageable computation cost.

==> Makefile <==
FILE_NAME := paper

TEMP_FILES := \
	$(FILE_NAME).aux \
	$(FILE_NAME).bbl \
	$(FILE_NAME).log \
	$(FILE_NAME).blg \
	$(FILE_NAME).brf \
	$(FILE_NAME).out

SECTION_FILES = \
	paper.tex \
	Sections/approach.tex \
	Sections/background.tex \
	Sections/introduction.tex \
	Sections/motivating-analysis.tex \
	Sections/results.tex \
	Sections/setup.tex

BIBTEX_FILES = \
	filteredref.bib 

GEN_FIGURES = \
	$(NULL)

# STATIC_FIGURES = \
# 	figure/overview.pdf 

DEBUG=no
ifneq '$(DEBUG)' 'yes'
LATEX_FLAGS="-interaction=batchmode"
endif

.DELETE_ON_ERROR:

################################################################################
# Main paper building
################################################################################
# $(STATIC_FIGURES)
$(FILE_NAME).pdf: $(SECTION_FILES) $(GEN_FIGURES) $(BIBTEX_FILES) 
	pdflatex $(LATEX_FLAGS) $(FILE_NAME)
	bibtex $(FILE_NAME)
	pdflatex $(LATEX_FLAGS) $(FILE_NAME)
	pdflatex $(LATEX_FLAGS) $(FILE_NAME)
	rm -f $(TEMP_FILES)
	# open $(FILE_NAME).pdf
	# rm $(FILE_NAME).pdf


################################################################################
# Camera-Ready
################################################################################
.PHONY: camera
camera: 
	pdftops $(FILE_NAME).pdf
	ps2pdf14 -dPDFSETTINGS=/prepress $(FILE_NAME).pdf $(FILE_NAME)-new.pdf
	# pdffont $(FILE_NAME).pdf
	mv $(FILE_NAME)-new.pdf $(FILE_NAME).pdf
	# open $(FILE_NAME).pdf
	# rm $(FILE_NAME).pdf
	
################################################################################
# Figures
################################################################################

#$(GEN_FIGURES): %.pdf: scripts/rms/analysis_figures.r scripts/rms/util.r
#	Rscript $<

################################################################################
# Clean
################################################################################
.PHONY: clean
clean:
	rm -f $(TEMP_FILES) $(GEN_FIGURES) $(FILE_NAME).pdf


==> Sections/ZZmotivating-analysis.tex <==

\section{Motivating Analysis}\label{sec:motivation}

In this section, we perform motivating analyses in order to better understand how much effort that developers could waste on localizing defective lines and how effective is line-level defect prediction.

\subsection*{(MA1) How much effort that developers could waste on localizing defective lines when using file-level defect prediction?}


\smallsection{Approach} 
We hypothesize that the proportion of defective lines in a file is relatively small. 
Hence, it is possible that developers may waste their effort in identifying defects by inspecting the whole file.
To perform our motivating analysis 1, we analyze our line-level defect datasets that are extracted from Version Control Systems and Issue Tracking Systems (see Figure \ref{fig:overview}).
We describe our approach of constructing line-level defect datasets in Section \ref{sec:construct_defect_data}.
Then, we examine the proportion of lines that are defective (i.e., $\frac{\#DefectiveLines}{LOC}$) of each file in the nine studied software systems.

\smallsection{Results} 
\textbf{As expected, as little as 1\% - 2.2\% of the lines of code of a file are defective, suggesting that developers could waste more than 98\% of SQA effort on localizing defective lines.}
Figure~\ref{fig:preliminary} presents the distribution of the proportion of defective lines of each file.
We find that at the median values, the proportion of defective lines in the defective files ranges from 1\% to 2.2\% across the nine studied software systems.
In addition, there are 30\% of defective files that have only one single defective line.
\emph{This finding suggests that a defect prediction framework to localize  defective lines is critically needed.}
% \kla{need an example figure}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{Figure/preliminary.png}
\label{fig:preliminary}
\caption{The ratio of defective lines in our defect datasets \asia{will be fixed} \protect\centering}
\end{figure}


==> Sections/bio.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio_pictures/asia.jpg}}]{Supatsara Wattanakriengkrai}
is a Master's student at the Department of Information Science, Nara Institute of Science and Technology, Japan.
She received her BS degree in Information and Communication Technology from Mahidol University, Thailand, in 2019. Her main research interests are Empirical Software Engineering, Mining Software Repositories, and Software Quality Assurance. Contact her at wattanakri.supatsara.ws3@is.naist.jp.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,trim=0 1000 200 400, clip,keepaspectratio]{bio_pictures/patanamon.jpg}}]{Patanamon Thongtanunam}
is a lecturer at the School of Computing and Information Systems, the University of Melbourne, Australia. 
% Prior to that, she was a research fellow of Japan Society for the Promotion of Science (JSPS). 
She received PhD in Information Science from Nara Institute of Science and Technology, Japan.
Her research interests include empirical software engineering, mining software repositories, software quality, and human aspect. Her research has been published at top-tier software engineering venues like International Conference on Software Engineering (ICSE) and Journal of Transaction on Software Engineering (TSE). 
More about Patanamon and her work is available online at 
\url{http://patanamon.com}.
\end{IEEEbiography}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio_pictures/kla.jpg}}]{Chakkrit Tantithamthavorn}
is a 2020 ARC DECRA Fellow and a Lecturer in Software Engineering in the Faculty of Information Technology, Monash University, Melbourne, Australia. 
His current fellowship is focusing on the development of ``Practical and Explainable Analytics to Prevent Future Software Defects''.
His work has been published at several top-tier software engineering venues, such as the IEEE Transactions on Software Engineering (TSE), the Springer Journal of Empirical Software Engineering (EMSE) and the International Conference on Software Engineering (ICSE). 
More about Chakkrit and his work is available online at \url{http://chakkrit.com}.
\end{IEEEbiography}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1in,clip,keepaspectratio]{bio_pictures/hata.jpg}}]{Hideaki Hata}
is an assistant professor at the Nara Institute of Science and Technology. His research interests include software ecosystems, human capital in software engineering, and software economics. He received a Ph.D. in information science from Osaka University.
More about Hideaki and his work is available online at \url{https://hideakihata.github.io/}.
\end{IEEEbiography}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio_pictures/matsumoto.png}}]{Kenichi Matsumoto}
is a professor in the Graduate School of Science and Technology at the Nara Institute of Science and Technology. His research interests include software measurement and software processes. He received a Ph.D. in information and computer sciences from Osaka University. He is a Senior Member of the IEEE and a member of the IEICE and the IPSJ. Contact him at matumoto@is.naist.jp.
\end{IEEEbiography}





